CheckerBench: Can Long-Horizon Agents Synthesize Static-Analysis Checkers?

Static-analysis checker synthesis requires agents to interpret a defect specification, inspect a repository, implement analyzer-specific logic, and refine the checker through repeated compilation and analysis feedback. Existing coding-agent benchmarks focus on tasks such as patch generation or vulnerability detection and rarely assess whether an agent can develop a working checker in a repository from start to finish. We introduce CheckerBench, an executable benchmark of 300 tasks derived from 297 CVEs across 167 repositories, 85 CWEs, and five language ecosystems. Each task includes vulnerable and fixed revisions, a pinned analysis environment, and a checker scaffold. We further introduce CheckerLab, a common evaluation framework that independently rebuilds submitted checkers and measures vulnerable-fixed diagnostic contrast, patch localization, false positives, and tool use. Across 21 model-harness configurations and three independent repeats per configuration, mean Pass@1 is 32.30%, while the best reaches 45.33%. These results show that reliable, reusable checker development remains challenging for current coding agents.

==> figures/logo/institution-logo-shadows.tex <==
% Soft shadows for the first-page institutional logos.
% The normalized outlines follow the artwork's visible bounds.
% Foreground PDF/PNG assets retain their original paths, lettering, and colors.
\newsavebox{\institutionlogobox}
\newcommand{\institutionlogoshadow}[2]{%
  \sbox{\institutionlogobox}{#2}%
  \begin{tikzpicture}[
    x=\wd\institutionlogobox,y=\ht\institutionlogobox,baseline=0pt]
    \path[use as bounding box] (0,0) rectangle (1,1);
    % Shadows do not change the logo's dimensions or the title layout.
    \begin{scope}[overlay]
      % Match the SII shadow in CoworkWorld's AffiliationLogo macro.
      \begin{scope}[xshift=0.85pt,yshift=-0.95pt,
          transparency group,opacity=0.32]
        \path[fill=black] #1;
        \foreach \shadowwidth/\shadowopacity in
            {2.4/0.015,2.0/0.035,1.6/0.055,1.2/0.095,0.8/0.15,0.4/0.25}{%
          \path[draw=black,line width=\shadowwidth pt,
            opacity=\shadowopacity,line join=round] #1;
        }
      \end{scope}
      \path[fill=white] #1;
      \begin{scope}[blend mode=multiply]
        % White bitmap margins reveal the shadow without clipping any artwork.
        \node[anchor=south west,inner sep=0pt,outer sep=0pt]
          at (0,0) {\usebox{\institutionlogobox}};
      \end{scope}
    \end{scope}
  \end{tikzpicture}%
}

\newcommand{\ecnulogosilhouette}{%
  (0.47345,0.96328) -- (0.55531,0.96328) -- (0.59292,0.95896) -- (0.62832,0.94816) --
  (0.64159,0.94816) -- (0.64602,0.94384) -- (0.65929,0.94384) -- (0.66150,0.93952) --
  (0.67478,0.93952) -- (0.67699,0.93521) -- (0.68805,0.93521) -- (0.69027,0.93089) --
  (0.70354,0.92873) -- (0.71018,0.92225) -- (0.72345,0.92009) -- (0.74115,0.90713) --
  (0.74779,0.90713) -- (0.75221,0.90065) -- (0.77434,0.89201) -- (0.82522,0.85529) --
  (0.86062,0.82505) -- (0.87168,0.80778) -- (0.87832,0.80562) -- (0.90265,0.77106) --
  (0.91593,0.76026) -- (0.92035,0.74730) -- (0.92920,0.74082) -- (0.92920,0.73434) --
  (0.94027,0.72138) -- (0.94027,0.71490) -- (0.95354,0.69546) -- (0.95354,0.68467) --
  (0.96460,0.67387) -- (0.96460,0.66307) -- (0.97788,0.64147) -- (0.98009,0.61987) --
  (0.98673,0.61123) -- (0.98894,0.58099) -- (0.99336,0.57883) -- (0.99336,0.56371) --
  (0.99779,0.55940) -- (1.00000,0.53132) -- (0.99779,0.42117) -- (0.99336,0.41685) --
  (0.99336,0.39741) -- (0.97788,0.34341) -- (0.97345,0.34125) -- (0.97345,0.33045) --
  (0.96460,0.31749) -- (0.96460,0.30670) -- (0.95354,0.29806) -- (0.95354,0.28726) --
  (0.93584,0.25486) -- (0.90708,0.21166) -- (0.90044,0.20950) -- (0.89381,0.19438) --
  (0.84735,0.14471) -- (0.82080,0.12743) -- (0.82080,0.12311) -- (0.80310,0.10799) --
  (0.78540,0.10151) -- (0.77434,0.08855) -- (0.74779,0.07991) -- (0.72124,0.06048) --
  (0.71239,0.06048) -- (0.70354,0.05184) -- (0.67035,0.04536) -- (0.65929,0.03672) --
  (0.64602,0.03672) -- (0.64381,0.03240) -- (0.54646,0.01728) -- (0.49115,0.01728) --
  (0.42478,0.02376) -- (0.42257,0.02808) -- (0.39602,0.03240) -- (0.39159,0.03672) --
  (0.35841,0.04104) -- (0.35177,0.04752) -- (0.31858,0.05616) -- (0.31637,0.06048) --
  (0.29204,0.06911) -- (0.28319,0.07991) -- (0.27212,0.07991) -- (0.26770,0.08639) --
  (0.25664,0.08855) -- (0.24336,0.10151) -- (0.21903,0.11231) -- (0.19690,0.13607) --
  (0.19027,0.13607) -- (0.18805,0.14471) -- (0.18142,0.14471) -- (0.17478,0.15551) --
  (0.15929,0.16631) -- (0.15929,0.17279) -- (0.15265,0.17279) -- (0.14602,0.17927) --
  (0.14159,0.19222) -- (0.12611,0.20302) -- (0.12611,0.20950) -- (0.10177,0.23758) --
  (0.10177,0.24622) -- (0.09292,0.25270) -- (0.09071,0.26782) -- (0.08186,0.27430) --
  (0.06858,0.29806) -- (0.06637,0.31317) -- (0.05973,0.31965) -- (0.05310,0.34773) --
  (0.04867,0.34989) -- (0.04867,0.36069) -- (0.04425,0.36285) -- (0.04425,0.37581) --
  (0.03982,0.37797) -- (0.02655,0.46004) -- (0.02655,0.53132) -- (0.03097,0.53996) --
  (0.03097,0.56371) -- (0.03540,0.56587) -- (0.03540,0.58747) -- (0.03982,0.58963) --
  (0.03982,0.60475) -- (0.05973,0.65443) -- (0.05973,0.66523) -- (0.07301,0.68467) --
  (0.07743,0.70194) -- (0.09071,0.71706) -- (0.09292,0.73002) -- (0.12611,0.77754) --
  (0.14381,0.79266) -- (0.14602,0.80130) -- (0.15708,0.80778) -- (0.18584,0.84017) --
  (0.21018,0.85529) -- (0.23451,0.87905) -- (0.24115,0.87905) -- (0.25664,0.89201) --
  (0.28982,0.90713) -- (0.29646,0.91577) -- (0.32080,0.92009) -- (0.32522,0.92657) --
  (0.34071,0.93089) -- (0.34292,0.93521) -- (0.35398,0.93521) -- (0.35619,0.93952) --
  (0.38274,0.94384) -- (0.40265,0.95248) -- (0.46681,0.95896) -- cycle%
}

\newcommand{\humanlayalogosilhouette}{%
  (0.50984,1.00000) -- (0.51699,1.00000) -- (0.52236,0.97523) -- (0.53131,0.96904) --
  (0.53309,0.94427) -- (0.54025,0.94118) -- (0.55098,0.91950) -- (0.55456,0.89164) --
  (0.56887,0.86687) -- (0.56887,0.85759) -- (0.58497,0.83282) -- (0.58676,0.80805) --
  (0.59928,0.79257) -- (0.60465,0.76780) -- (0.62612,0.72136) -- (0.62791,0.70588) --
  (0.63864,0.69040) -- (0.63864,0.66873) -- (0.64401,0.66873) -- (0.65474,0.65325) --
  (0.66547,0.60681) -- (0.67442,0.59133) -- (0.67621,0.57895) -- (0.69231,0.55728) --
  (0.69231,0.54180) -- (0.69767,0.53870) -- (0.70483,0.50464) -- (0.72451,0.46749) --
  (0.73882,0.47368) -- (0.74419,0.49536) -- (0.75492,0.50155) -- (0.77102,0.52632) --
  (0.78175,0.52941) -- (0.79785,0.52322) -- (0.79785,0.49845) -- (0.80143,0.50155) --
  (0.81038,0.48916) -- (0.81574,0.45511) -- (0.83005,0.44582) -- (0.83363,0.41176) --
  (0.84973,0.39009) -- (0.85152,0.35913) -- (0.86047,0.35913) -- (0.86404,0.35294) --
  (0.86762,0.33127) -- (0.87835,0.31579) -- (0.89445,0.26935) -- (0.90161,0.26316) --
  (0.90519,0.22910) -- (0.92129,0.21053) -- (0.93023,0.17647) -- (0.93381,0.17647) --
  (0.94097,0.15170) -- (0.95349,0.13622) -- (0.95707,0.12693) -- (0.95707,0.10836) --
  (0.96243,0.10526) -- (0.97496,0.07740) -- (0.97674,0.05263) -- (0.99463,0.02786) --
  (0.99463,0.01238) -- (0.98211,0.00000) -- (0.74240,0.00310) -- (0.71020,0.01238) --
  (0.70662,0.04334) -- (0.71199,0.07740) -- (0.71556,0.08050) -- (0.71556,0.10836) --
  (0.72451,0.14861) -- (0.72451,0.17028) -- (0.72809,0.17337) -- (0.72809,0.20743) --
  (0.74061,0.25077) -- (0.74419,0.24768) -- (0.74597,0.17337) -- (0.75134,0.17028) --
  (0.75492,0.08978) -- (0.76208,0.07430) -- (0.76208,0.06502) -- (0.76923,0.05882) --
  (0.85510,0.05882) -- (0.86225,0.05263) -- (0.88014,0.05263) -- (0.88372,0.05882) --
  (0.88193,0.07740) -- (0.87299,0.07740) -- (0.86047,0.08978) -- (0.79606,0.08978) --
  (0.79428,0.09598) -- (0.77818,0.09288) -- (0.77460,0.09907) -- (0.76744,0.13313) --
  (0.76744,0.18885) -- (0.76029,0.23529) -- (0.76029,0.26006) -- (0.75492,0.26625) --
  (0.75134,0.35604) -- (0.74240,0.37461) -- (0.73703,0.37461) -- (0.72809,0.35604) --
  (0.72809,0.30960) -- (0.71735,0.26316) -- (0.71556,0.21672) -- (0.71199,0.21053) --
  (0.71020,0.17337) -- (0.70483,0.17028) -- (0.69946,0.08669) -- (0.69589,0.07740) --
  (0.68515,0.07740) -- (0.68157,0.08359) -- (0.68157,0.12693) -- (0.67800,0.13003) --
  (0.67621,0.17028) -- (0.66905,0.17957) -- (0.66547,0.19814) -- (0.65653,0.17337) --
  (0.64937,0.16718) -- (0.64758,0.14551) -- (0.63864,0.13313) -- (0.63864,0.10217) --
  (0.63506,0.09288) -- (0.60465,0.08669) -- (0.53131,0.08978) -- (0.52415,0.07740) --
  (0.51878,0.07740) -- (0.51878,0.06502) -- (0.52594,0.05882) -- (0.63685,0.05882) --
  (0.64580,0.06502) -- (0.65295,0.10526) -- (0.66369,0.11146) -- (0.66726,0.08978) --
  (0.67442,0.07430) -- (0.67442,0.01858) -- (0.66726,0.00619) -- (0.45259,0.00310) --
  (0.43649,0.01238) -- (0.43292,0.02786) -- (0.44544,0.05573) -- (0.44902,0.07740) --
  (0.45617,0.08359) -- (0.45617,0.09907) -- (0.46333,0.11146) -- (0.46333,0.12074) --
  (0.47585,0.13313) -- (0.47585,0.15789) -- (0.48122,0.17028) -- (0.49195,0.17647) --
  (0.59034,0.17647) -- (0.59928,0.21672) -- (0.60286,0.25697) -- (0.60823,0.26625) --
  (0.61002,0.33746) -- (0.61717,0.35913) -- (0.61538,0.40248) -- (0.62970,0.42724) --
  (0.63685,0.42724) -- (0.63864,0.42105) -- (0.65116,0.42724) -- (0.65295,0.44272) --
  (0.64580,0.44892) -- (0.64580,0.46440) -- (0.64043,0.46749) -- (0.63506,0.48297) --
  (0.63506,0.50774) -- (0.63148,0.50774) -- (0.61181,0.54799) -- (0.61181,0.56656) --
  (0.60823,0.56966) -- (0.59928,0.61920) -- (0.59571,0.69969) -- (0.59213,0.70279) --
  (0.59034,0.71827) -- (0.58140,0.72446) -- (0.58140,0.74923) -- (0.55098,0.78019) --
  (0.54204,0.79567) -- (0.53309,0.79876) -- (0.52952,0.81115) -- (0.50805,0.81115) --
  (0.50626,0.78328) -- (0.49195,0.75542) -- (0.48837,0.72446) -- (0.47943,0.72136) --
  (0.47943,0.69350) -- (0.46512,0.67183) -- (0.45975,0.63158) -- (0.45259,0.62848) --
  (0.45259,0.61300) -- (0.44007,0.58824) -- (0.43292,0.54489) -- (0.44544,0.54489) --
  (0.44544,0.55728) -- (0.45796,0.57895) -- (0.46512,0.60372) -- (0.47585,0.61610) --
  (0.47585,0.62539) -- (0.48122,0.63467) -- (0.48837,0.63467) -- (0.49195,0.65325) --
  (0.50089,0.66563) -- (0.51342,0.66254) -- (0.52594,0.63467) -- (0.53309,0.63158) --
  (0.53309,0.61300) -- (0.54204,0.60062) -- (0.54204,0.56966) -- (0.53309,0.55728) --
  (0.53309,0.54180) -- (0.52236,0.53251) -- (0.51163,0.50155) -- (0.49016,0.46440) --
  (0.48837,0.44892) -- (0.47943,0.44582) -- (0.47943,0.43344) -- (0.44186,0.37152) --
  (0.43828,0.35294) -- (0.42755,0.34985) -- (0.42576,0.32817) -- (0.41324,0.31269) --
  (0.40966,0.29721) -- (0.39893,0.28173) -- (0.39714,0.26935) -- (0.37925,0.23529) --
  (0.37388,0.23220) -- (0.37209,0.21672) -- (0.35420,0.19505) -- (0.35063,0.17337) --
  (0.33989,0.16718) -- (0.33631,0.14861) -- (0.32737,0.13313) -- (0.32021,0.13003) --
  (0.31843,0.10836) -- (0.30948,0.10526) -- (0.30233,0.09288) -- (0.30233,0.08050) --
  (0.29338,0.07430) -- (0.28980,0.05573) -- (0.28086,0.04025) -- (0.26655,0.02786) --
  (0.26476,0.01238) -- (0.23971,0.00310) -- (0.02147,0.00310) -- (0.00894,0.00929) --
  (0.00358,0.02167) -- (0.01968,0.05263) -- (0.02326,0.07740) -- (0.03041,0.08359) --
  (0.03399,0.10217) -- (0.05009,0.12384) -- (0.05009,0.14241) -- (0.06082,0.15789) --
  (0.06082,0.16718) -- (0.08408,0.21362) -- (0.08945,0.23529) -- (0.10197,0.24458) --
  (0.10376,0.27245) -- (0.11986,0.30031) -- (0.12343,0.31579) -- (0.13059,0.32198) --
  (0.14311,0.36842) -- (0.15564,0.38390) -- (0.15921,0.40867) -- (0.17352,0.42724) --
  (0.17710,0.44892) -- (0.18426,0.45511) -- (0.20036,0.50464) -- (0.20930,0.51393) --
  (0.20930,0.53251) -- (0.21467,0.54180) -- (0.22361,0.54489) -- (0.22361,0.56037) --
  (0.24150,0.59752) -- (0.25045,0.63158) -- (0.26297,0.63467) -- (0.26297,0.65944) --
  (0.27907,0.68111) -- (0.28623,0.71827) -- (0.29159,0.72755) -- (0.30233,0.72755) --
  (0.30590,0.73684) -- (0.31485,0.73994) -- (0.31843,0.72446) -- (0.32558,0.72136) --
  (0.34705,0.66873) -- (0.35420,0.65944) -- (0.36852,0.66254) -- (0.37030,0.69040) --
  (0.38640,0.71207) -- (0.38640,0.72446) -- (0.40250,0.75232) -- (0.40966,0.78019) --
  (0.42218,0.79257) -- (0.42218,0.81115) -- (0.43649,0.82043) -- (0.44544,0.85449) --
  (0.45796,0.87616) -- (0.46512,0.90093) -- (0.47764,0.91331) -- (0.48301,0.93808) --
  (0.49911,0.96285) -- (0.50447,0.99381) -- cycle%
}

\newcommand{\sjtulogosilhouette}{%
  (0.45309,0.96328) -- (0.54920,0.96328) -- (0.64073,0.94816) -- (0.64302,0.94384) --
  (0.66819,0.93952) -- (0.70709,0.92009) -- (0.71625,0.92009) -- (0.73455,0.90713) --
  (0.74371,0.90713) -- (0.74828,0.90065) -- (0.77117,0.89201) -- (0.78490,0.87905) --
  (0.81236,0.86393) -- (0.82380,0.85097) -- (0.83753,0.84449) -- (0.88101,0.79914) --
  (0.88787,0.79698) -- (0.89245,0.78618) -- (0.91762,0.75810) -- (0.91762,0.75162) --
  (0.92449,0.74946) -- (0.92449,0.74298) -- (0.94279,0.72138) -- (0.94279,0.71490) --
  (0.96796,0.67387) -- (0.97254,0.65011) -- (0.98398,0.63283) -- (0.98627,0.59827) --
  (0.99314,0.59611) -- (0.99771,0.58315) -- (1.00000,0.41685) -- (0.97712,0.33045) --
  (0.97254,0.32829) -- (0.96796,0.30670) -- (0.95195,0.28294) -- (0.95195,0.27646) --
  (0.95881,0.27214) -- (0.95195,0.26998) -- (0.95195,0.27646) -- (0.94737,0.27430) --
  (0.94279,0.25918) -- (0.93364,0.25270) -- (0.92449,0.23110) -- (0.90389,0.20950) --
  (0.90389,0.20302) -- (0.85584,0.15551) -- (0.85584,0.15119) -- (0.78719,0.09719) --
  (0.78032,0.09719) -- (0.74600,0.07343) -- (0.68650,0.04752) -- (0.65675,0.04104) --
  (0.64302,0.03240) -- (0.57437,0.01944) -- (0.45995,0.01728) -- (0.40503,0.02376) --
  (0.40046,0.02808) -- (0.38444,0.02808) -- (0.36613,0.03672) -- (0.35469,0.03672) --
  (0.35240,0.04104) -- (0.34096,0.04104) -- (0.33867,0.04536) -- (0.31808,0.05184) --
  (0.30664,0.05184) -- (0.29748,0.06048) -- (0.28833,0.06048) -- (0.28604,0.06479) --
  (0.26087,0.07343) -- (0.25629,0.07991) -- (0.24714,0.07991) -- (0.24027,0.08639) --
  (0.23570,0.08423) -- (0.23341,0.09287) -- (0.20824,0.10367) -- (0.19680,0.11663) --
  (0.17162,0.13175) -- (0.16476,0.13823) -- (0.16476,0.14471) -- (0.15789,0.14471) --
  (0.14645,0.15335) -- (0.14645,0.15767) -- (0.10069,0.20302) -- (0.09611,0.21598) --
  (0.06636,0.25054) -- (0.06636,0.25702) -- (0.03661,0.30670) -- (0.03204,0.32613) --
  (0.02746,0.32829) -- (0.02517,0.34773) -- (0.01831,0.35205) -- (0.00229,0.41469) --
  (0.00000,0.53132) -- (0.00229,0.56371) -- (0.00686,0.56803) -- (0.00686,0.58531) --
  (0.01144,0.58747) -- (0.01373,0.61339) -- (0.02746,0.64363) -- (0.02746,0.65875) --
  (0.03661,0.66523) -- (0.04805,0.69978) -- (0.05721,0.70842) -- (0.06636,0.73218) --
  (0.07780,0.74082) -- (0.07780,0.74730) -- (0.09611,0.77322) -- (0.17849,0.85529) --
  (0.27231,0.91577) -- (0.29977,0.92009) -- (0.30435,0.92873) -- (0.32265,0.93089) --
  (0.34783,0.94384) -- (0.36156,0.94384) -- (0.36384,0.94816) -- cycle%
}

\newcommand{\pkulogosilhouette}{%
  (0.45205,0.96537) -- (0.55936,0.96537) -- (0.60274,0.95887) -- (0.62557,0.95022) --
  (0.64155,0.95022) -- (0.65753,0.94156) -- (0.69178,0.93290) -- (0.70091,0.92208) --
  (0.71233,0.92424) -- (0.73059,0.91775) -- (0.73744,0.90909) -- (0.74429,0.90909) --
  (0.74886,0.90260) -- (0.75571,0.90260) -- (0.76256,0.89394) -- (0.76941,0.89394) --
  (0.79909,0.87446) -- (0.86986,0.81385) -- (0.87443,0.80303) -- (0.89498,0.78571) --
  (0.89954,0.77489) -- (0.92009,0.75325) -- (0.92009,0.74675) -- (0.93379,0.72727) --
  (0.94064,0.72294) -- (0.97489,0.64935) -- (0.97489,0.63853) -- (0.97945,0.63636) --
  (1.00000,0.55195) -- (1.00000,0.43723) -- (0.99543,0.42857) -- (0.99543,0.40909) --
  (0.98858,0.40260) -- (0.98858,0.37446) -- (0.97945,0.36147) -- (0.97945,0.34848) --
  (0.96347,0.31602) -- (0.96347,0.30736) -- (0.95890,0.30519) -- (0.95890,0.29654) --
  (0.93379,0.25758) -- (0.93379,0.25108) -- (0.92009,0.24026) -- (0.92009,0.23160) --
  (0.89954,0.20996) -- (0.89954,0.20346) -- (0.88584,0.19264) -- (0.86530,0.16450) --
  (0.85160,0.15584) -- (0.84703,0.14502) -- (0.83790,0.14502) -- (0.83562,0.13853) --
  (0.81050,0.11688) -- (0.78539,0.10390) -- (0.76941,0.08874) -- (0.76256,0.08874) --
  (0.75571,0.08009) -- (0.74201,0.08009) -- (0.73516,0.06926) -- (0.72603,0.06926) --
  (0.72374,0.06494) -- (0.66667,0.04113) -- (0.60274,0.02814) -- (0.59817,0.02381) --
  (0.57763,0.02381) -- (0.55251,0.01732) -- (0.45890,0.01732) -- (0.37900,0.02814) --
  (0.37671,0.03247) -- (0.36301,0.03247) -- (0.36073,0.03680) -- (0.34932,0.03680) --
  (0.33562,0.04545) -- (0.32420,0.04545) -- (0.30365,0.05628) -- (0.29452,0.05628) --
  (0.29224,0.06061) -- (0.26712,0.06926) -- (0.25571,0.08009) -- (0.24429,0.08225) --
  (0.23973,0.07792) -- (0.23744,0.08874) -- (0.23059,0.08874) -- (0.20776,0.10823) --
  (0.18950,0.11688) -- (0.16895,0.13420) -- (0.16667,0.14286) -- (0.15753,0.14502) --
  (0.12785,0.17100) -- (0.12100,0.18398) -- (0.10502,0.19481) -- (0.10046,0.20996) --
  (0.07534,0.23810) -- (0.05936,0.27056) -- (0.05023,0.27706) -- (0.04338,0.29870) --
  (0.03425,0.30736) -- (0.03196,0.33766) -- (0.02283,0.34199) -- (0.02055,0.35931) --
  (0.01598,0.36147) -- (0.00000,0.43723) -- (0.00000,0.54545) -- (0.00228,0.56277) --
  (0.00685,0.56710) -- (0.01142,0.61039) -- (0.02055,0.62554) -- (0.02055,0.63853) --
  (0.03196,0.65368) -- (0.03196,0.66883) -- (0.04566,0.68831) -- (0.06621,0.73377) --
  (0.08447,0.75325) -- (0.09132,0.77056) -- (0.10046,0.77489) -- (0.11187,0.79221) --
  (0.11644,0.79221) -- (0.12100,0.80519) -- (0.13014,0.80952) -- (0.16438,0.84632) --
  (0.17580,0.85065) -- (0.18721,0.86580) -- (0.19406,0.86580) -- (0.21689,0.88528) --
  (0.24886,0.90043) -- (0.25571,0.90909) -- (0.27397,0.91342) -- (0.28311,0.92208) --
  (0.30365,0.92208) -- (0.30594,0.93074) -- (0.34247,0.94156) -- (0.34475,0.94589) -- cycle%
}

\newcommand{\siilogosilhouette}{%
  (0.88603,0.94805) -- (0.91912,0.94805) -- (0.93015,0.93939) -- (0.93015,0.88745) --
  (0.95221,0.85498) -- (0.96324,0.85498) -- (0.97059,0.84199) -- (1.00000,0.82684) --
  (1.00000,0.75758) -- (0.95588,0.72944) -- (0.93382,0.72294) -- (0.91912,0.71212) --
  (0.88971,0.70563) -- (0.88235,0.69264) -- (0.85662,0.68831) -- (0.84191,0.67532) --
  (0.82353,0.67100) -- (0.80515,0.65801) -- (0.77941,0.65801) -- (0.77574,0.64502) --
  (0.76103,0.64286) -- (0.73897,0.62554) -- (0.71324,0.62121) -- (0.69485,0.60606) --
  (0.67279,0.60173) -- (0.66912,0.59524) -- (0.65441,0.59307) -- (0.64338,0.58442) --
  (0.64706,0.58009) -- (0.66544,0.57792) -- (0.66912,0.56926) -- (0.68382,0.56926) --
  (0.73897,0.54978) -- (0.76838,0.54545) -- (0.77941,0.53896) -- (0.77941,0.53247) --
  (0.80882,0.53247) -- (0.81250,0.52165) -- (0.85294,0.49567) -- (0.86029,0.46753) --
  (0.84559,0.46320) -- (0.84191,0.45455) -- (0.83088,0.45238) -- (0.79044,0.42424) --
  (0.77941,0.42424) -- (0.77206,0.41558) -- (0.75735,0.41558) -- (0.74265,0.40043) --
  (0.72059,0.40043) -- (0.72059,0.39394) -- (0.70588,0.38312) -- (0.66912,0.37446) --
  (0.66544,0.36797) -- (0.63603,0.36797) -- (0.60294,0.33550) -- (0.58824,0.33550) --
  (0.55147,0.30952) -- (0.53676,0.30736) -- (0.48529,0.28355) -- (0.47426,0.27273) --
  (0.45221,0.27273) -- (0.44853,0.25974) -- (0.42647,0.25541) -- (0.40809,0.24026) --
  (0.39706,0.24026) -- (0.36029,0.21861) -- (0.34191,0.21645) -- (0.34191,0.20996) --
  (0.31985,0.20563) -- (0.30515,0.19048) -- (0.27574,0.18182) -- (0.24265,0.16234) --
  (0.23162,0.16234) -- (0.20956,0.14502) -- (0.18750,0.14286) -- (0.18382,0.13420) --
  (0.16176,0.12338) -- (0.13971,0.11472) -- (0.12500,0.11472) -- (0.12500,0.10823) --
  (0.08456,0.09307) -- (0.07721,0.08225) -- (0.05515,0.07792) -- (0.05515,0.06710) --
  (0.04044,0.05844) -- (0.04044,0.05195) -- (0.02941,0.04329) -- (0.01471,0.04113) --
  (0.00368,0.05628) -- (0.00735,0.28571) -- (0.05882,0.32035) -- (0.07353,0.32251) --
  (0.08456,0.33550) -- (0.09559,0.33983) -- (0.11765,0.33983) -- (0.11765,0.34848) --
  (0.13235,0.35714) -- (0.20221,0.39177) -- (0.22426,0.39610) -- (0.22426,0.40260) --
  (0.24632,0.40693) -- (0.27206,0.42424) -- (0.30882,0.43939) -- (0.33088,0.44156) --
  (0.33456,0.45455) -- (0.34926,0.45671) -- (0.36029,0.46537) -- (0.34559,0.46753) --
  (0.33456,0.47619) -- (0.29412,0.48052) -- (0.26471,0.49351) -- (0.23529,0.49567) --
  (0.22426,0.50433) -- (0.18750,0.50866) -- (0.18382,0.51299) -- (0.15809,0.51732) --
  (0.14338,0.52814) -- (0.11765,0.52814) -- (0.08456,0.54113) -- (0.04779,0.54545) --
  (0.01471,0.56494) -- (0.00735,0.57143) -- (0.00368,0.59524) -- (0.00735,0.72078) --
  (0.05147,0.75325) -- (0.08824,0.76623) -- (0.11765,0.76407) -- (0.13235,0.77056) --
  (0.16912,0.77056) -- (0.18015,0.77489) -- (0.55515,0.77273) -- (0.55882,0.77922) --
  (0.57721,0.78139) -- (0.58824,0.79004) -- (0.60662,0.79004) -- (0.61029,0.79870) --
  (0.63235,0.81385) -- (0.66176,0.81818) -- (0.66176,0.82900) -- (0.68750,0.83550) --
  (0.70588,0.85498) -- (0.72426,0.85498) -- (0.74632,0.87229) -- (0.77206,0.87879) --
  (0.77206,0.88528) -- (0.80515,0.89827) -- (0.83824,0.91991) -- (0.85294,0.91991) --
  (0.86029,0.93074) -- (0.88235,0.93723) -- cycle%
}


==> sections/float-placement.tex <==
% Save the template defaults so these adjustments apply only to the main text.
\makeatletter
\edef\restorefloatlayout{%
  \noexpand\floatplacement{figure}{\fps@figure}%
  \noexpand\floatplacement{table}{\fps@table}%
  \noexpand\setcounter{topnumber}{\number\c@topnumber}%
  \noexpand\setcounter{bottomnumber}{\number\c@bottomnumber}%
  \noexpand\setcounter{totalnumber}{\number\c@totalnumber}%
  \noexpand\setcounter{dbltopnumber}{\number\c@dbltopnumber}%
  \noexpand\renewcommand{\noexpand\topfraction}{\topfraction}%
  \noexpand\renewcommand{\noexpand\bottomfraction}{\bottomfraction}%
  \noexpand\renewcommand{\noexpand\dbltopfraction}{\dbltopfraction}%
  \noexpand\renewcommand{\noexpand\textfraction}{\textfraction}%
  \noexpand\renewcommand{\noexpand\floatpagefraction}{\floatpagefraction}%
  \noexpand\renewcommand{\noexpand\dblfloatpagefraction}{\dblfloatpagefraction}%
  \noexpand\setlength{\noexpand\textfloatsep}{\the\textfloatsep}%
  \noexpand\setlength{\noexpand\floatsep}{\the\floatsep}%
  \noexpand\setlength{\noexpand\dbltextfloatsep}{\the\dbltextfloatsep}%
  \noexpand\setlength{\noexpand\dblfloatsep}{\the\dblfloatsep}%
  \noexpand\setlength{\noexpand\parskip}{\the\parskip}%
  \noexpand\def\noexpand\ftype@table{\ftype@table}%
  \noexpand\setlength{\noexpand\@fptop}{\the\@fptop}%
  \noexpand\setlength{\noexpand\@fpsep}{\the\@fpsep}%
  \noexpand\setlength{\noexpand\@fpbot}{\the\@fpbot}%
  \noexpand\setlength{\noexpand\@dblfptop}{\the\@dblfptop}%
  \noexpand\setlength{\noexpand\@dblfpsep}{\the\@dblfpsep}%
  \noexpand\setlength{\noexpand\@dblfpbot}{\the\@dblfpbot}%
}
\makeatother

% Keep floats close to the discussion while leaving room for prose below.
% Figure 1 remains inline on the title page. Prefer page tops; the ablation
% table may use the bottom to follow the preceding inline comparison table.
\floatplacement{figure}{tp}
\floatplacement{table}{tp}
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{1}
\setcounter{totalnumber}{2}
\setcounter{dbltopnumber}{2}
\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.35}
\renewcommand{\dbltopfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.85}
\renewcommand{\dblfloatpagefraction}{0.85}
\setlength{\textfloatsep}{12pt plus 2pt minus 2pt}
\setlength{\floatsep}{10pt plus 2pt minus 2pt}
\setlength{\dbltextfloatsep}{12pt plus 2pt minus 2pt}
\setlength{\dblfloatsep}{10pt plus 2pt minus 2pt}

% Top-align float-only pages, with normal spacing between consecutive items.
\makeatletter
% Share the float ordering class so tables cannot overtake earlier figures.
% Caption names and counters remain separate. No per-float page break is needed.
\let\ftype@table\ftype@figure
\setlength{\@fptop}{0pt}
\setlength{\@fpsep}{12pt}
\setlength{\@fpbot}{0pt plus 1fil}
\setlength{\@dblfptop}{0pt}
\setlength{\@dblfpsep}{12pt}
\setlength{\@dblfpbot}{0pt plus 1fil}
\makeatother

% Appendix long tables retain their own continuous-page layout.

